Measurement of the CP-violating phase $\phi_s$ and the $B^0_s$ meson decay width difference with $B^0_s \to J/\psi\phi$ decays in ATLAS

A measurement of the $B^0_s$ decay parameters in the $B^0_s \to J/\psi\phi$ channel using an integrated luminosity of 14.3 $\mathrm{fb}^{-1}$ collected by the ATLAS detector from 8 TeV $pp$ collisions at the LHC is presented. The measured parameters include the $CP$-violating phase $\phi_s$, the decay width $\Gamma_s$ and the width difference between the mass eigenstates $\Delta\Gamma_s$. The values measured for the physical parameters are statistically combined with those from 4.9 $\mathrm{fb}^{-1}$ of 7 TeV data, leading to the following: \begin{eqnarray*} \phi_s & = & -0.090 \pm 0.078\;\mathrm{(stat.)} \pm 0.041\;\mathrm{(syst.)\;rad} \\ \Delta\Gamma_s & = & 0.085 \pm 0.011\;\mathrm{(stat.)} \pm 0.007\;\mathrm{(syst.)\;ps}^{-1} \\ \Gamma_s & = & 0.675 \pm 0.003\;\mathrm{(stat.)} \pm 0.003\;\mathrm{(syst.)\;ps}^{-1}. \end{eqnarray*} In the analysis the parameter $\Delta\Gamma_s$ is constrained to be positive. Results for $\phi_s$ and $\Delta\Gamma_s$ are also presented as 68% and 95% likelihood contours in the $\phi_s-\Delta\Gamma_s$ plane. Also measured in this decay channel are the transversity amplitudes and corresponding strong phases. All measurements are in agreement with the Standard Model predictions.

==> keys.tex <==
\makeatletter
\newcommand*{\numtablerange}[1][]{%
  \kernel@ifnextchar[{\numtable@range{#1}}{\numtable@range{#1}[#1]}}

\def\numtable@range#1[#2]#3#4{%
  \numtablerange@boxme{\expandafter\tablenum\expandafter[\numtablerange@lopt, #1]{#3}} $\pm$
  \numtablerange@boxme{\expandafter\tablenum\expandafter[\numtablerange@ropt, #2]{#4}}
}
\newcolumntype{T}[3]{>{\def\numtablerange@lopt{#1}\def\numtablerange@ropt{#2}}#3}

\newcommand*{\numtablerange@boxme}[1]{{\sbox0{#1}\usebox0}}
\makeatletter

\newcommand{\ilumi} {$ 14.3\, \rm fb^{-1} $}
\newcommand{\CoMEnergy}{8~\TeV}
\newcommand{\CoMEnergySeven}{7~\TeV}

\newcommand{\kminus} {\Kminus}
\newcommand{\kplus} {\Kplus}

\newcommand{\ntotal} {\ensuremath{ 375987}} 
\newcommand{\ntotaltext} {375,987}

\ifthenelse {\boolean{BdFraction3.3}}
{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Default fit    August version  %%%%%%%%% - version Bd 3.3%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\Bdfrac} {\ensuremath{ (3.3 \pm 0.5)\%}}
\newcommand{\nsig} {\ensuremath{ 73695 \pm 378  }}

\newcommand{\pSfit}     {\ensuremath{-0.110 }}
\newcommand{\pSstat}    {\ensuremath{ 0.082 }}
%

\newcommand{\DGfit}     {\ensuremath{ 0.101 }}
\newcommand{\DGstat}   {\ensuremath{ 0.013 }}
%

\newcommand{\GSfit}    {\ensuremath{ 0.676 }}
\newcommand{\GSstat}    {\ensuremath{ 0.004 }}
%

\newcommand{\Apasqfit}    {\ensuremath{ 0.230 }}
\newcommand{\Apasqstat}  {\ensuremath{ 0.005 }}
%

\newcommand{\Azesqfit}    {\ensuremath{ 0.520 }}
\newcommand{\Azesqstat}    {\ensuremath{ 0.004 }}
%

\newcommand{\ASsqfit}     {\ensuremath{ 0.097 }}
\newcommand{\ASsqstat}     {\ensuremath{ 0.008 }}
%

\newcommand{\Deltparafit}    {\ensuremath{ 3.15 }}
\newcommand{\Deltparastat}    {\ensuremath{ 0.10 }}
%

\newcommand{\Deltperpfit}     {\ensuremath{ 4.50 }}
\newcommand{\Deltperpstat}    {\ensuremath{ 0.45 }}
%

\newcommand{\DeltPSfit}        {\ensuremath{ -0.08 }}
\newcommand{\DeltSstat}       {\ensuremath{ 0.03 }}  %0.035 


% phi
\newcommand{\pAz}    {\ensuremath{ 0.029 }}
\newcommand{\pApa}   {\ensuremath{ 0.030 }}
\newcommand{\pAs}   {\ensuremath{ 0.048 }}
\newcommand{\pG}    {\ensuremath{ -0.085 }}
\newcommand{\pDG}   {\ensuremath{ 0.097 }}
\newcommand{\pDpara}    {\ensuremath{ 0.067 }}
\newcommand{\pDperp}   {\ensuremath{ 0.035 }}
\newcommand{\pDpS}  {\ensuremath{ -0.008 }}
%

% DG
%

\newcommand{\DGAz}  {\ensuremath{ 0.136 }}
\newcommand{\DGApa}  {\ensuremath{ 0.098 }}
\newcommand{\DGAs}   {\ensuremath{ 0.045 }}
\newcommand{\DGG}   {\ensuremath{ -0.414 }}
\newcommand{\DGDpara}   {\ensuremath{ 0.009 }}
\newcommand{\DGDperp}  {\ensuremath{ 0.008 }}
\newcommand{\DGDpS}   {\ensuremath{ -0.011 }}
%

% G
\newcommand{\GAz}    {\ensuremath{ -0.042 }}
\newcommand{\GApa}  {\ensuremath{ -0.119 }}
\newcommand{\GAs}   {\ensuremath{ 0.167 }}
\newcommand{\GDpara}    {\ensuremath{ -0.027 }}
\newcommand{\GDperp}    {\ensuremath{ -0.009 }}
\newcommand{\GDpS}    {\ensuremath{ 0.018 }}
%

% Az
\newcommand{\AzApa}  {\ensuremath{ -0.330 }}
\newcommand{\AzAs}  {\ensuremath{ 0.234 }}
\newcommand{\AzDpara}    {\ensuremath{ -0.011 }}
\newcommand{\AzDperp}   {\ensuremath{ 0.007 }}
\newcommand{\AzDpS}    {\ensuremath{ 0.014 }}
%

% Apa
\newcommand{\ApaAs}  {\ensuremath{ 0.072 }}
\newcommand{\ApaDpara}    {\ensuremath{ 0.105 }}
\newcommand{\ApaDperp}    {\ensuremath{ 0.025 }}
\newcommand{\ApaDpS}    {\ensuremath{ -0.018 }}
%

% As
\newcommand{\AsDpara}    {\ensuremath{ -0.046 }}
\newcommand{\AsDperp}    {\ensuremath{  0.004 }}
\newcommand{\AsDpS}  {\ensuremath{ 0.052 }}
%

% DeltaPara
\newcommand{\DparaDperp}    {\ensuremath{ 0.158 }}
\newcommand{\DparaDpS}    {\ensuremath{ -0.006 }}
%

% DeltaPerp
\newcommand{\DperpDpS}    {\ensuremath{ 0.018 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                                          SYSTEMATICS August Bd3.3%                     %%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\pSsyst} { 0.042}
\newcommand{\DGsyst} { 0.007}
\newcommand{\GSsyst}  { 0.004}
\newcommand{\Apasqsyst} { 0.006}
\newcommand{\Azesqsyst} { 0.007}
\newcommand{\ASsqsyst}  { 0.022}
\newcommand{\Deltperpsyst} { 0.30} 
\newcommand{\Deltparasyst} { 0.05}
\newcommand{\DeltPSsyst}   { 0.01}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  End of  Default fit    August version  %%%%%%%%% - version Bd 3.3%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
}
{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Default fit    9 June version  %%%%%%%%% - version Bd 2.4%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\Bdfrac} {\ensuremath{ (2.4 \pm 0.2)\%}}
\newcommand{\nsig} {\ensuremath{ 75124 \pm 383  }} 
%  
\newcommand{\pSfit}     { \ensuremath{-0.119 }}
\newcommand{\pSstat}    { \ensuremath{0.088 }}
%

\newcommand{\DGfit}     { \ensuremath{0.096 }}
\newcommand{\DGstat}   { \ensuremath{0.013 }}
%

\newcommand{\GSfit}    { \ensuremath{0.679 }}
\newcommand{\GSstat}    { \ensuremath{0.004 }}
%

\newcommand{\Apasqfit}    { \ensuremath{0.230 }}
\newcommand{\Apasqstat}  { \ensuremath{0.005 }}
%

\newcommand{\Azesqfit}    { \ensuremath{0.514 }}
\newcommand{\Azesqstat}    { \ensuremath{0.004 }}
%

\newcommand{\ASsqfit}     { \ensuremath{0.093 }}
\newcommand{\ASsqstat}     { \ensuremath{0.008 }}
%

\newcommand{\Deltparafit}    { \ensuremath{3.16 }}
\newcommand{\Deltparastat}    { \ensuremath{0.13 }}
%

\newcommand{\Deltperpfit}     { \ensuremath{4.46 }}
\newcommand{\Deltperpstat}    { \ensuremath{0.49 }}
%

\newcommand{\DeltPSfit}        { \ensuremath{-0.08 }}
\newcommand{\DeltSstat}       { \ensuremath{0.03 }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        Correlations  default fit    9 June version                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% phi
\newcommand{\pAz}    { \ensuremath{0.030 }}
\newcommand{\pApa}   { \ensuremath{0.043 }}
\newcommand{\pAs}   { \ensuremath{0.046 }}
\newcommand{\pG}    { \ensuremath{-0.097 }}
\newcommand{\pDG}   { \ensuremath{0.110 }}
\newcommand{\pDpara}    { \ensuremath{0.093 }}
\newcommand{\pDperp}   { \ensuremath{0.034 }}
\newcommand{\pDpS}  { \ensuremath{-0.001 }}
%

% DG
%

\newcommand{\DGAz}  { \ensuremath{0.139 }}
\newcommand{\DGApa}  { \ensuremath{0.104 }}
\newcommand{\DGAs}   { \ensuremath{0.051 }}
\newcommand{\DGG}   { \ensuremath{-0.421 }}
\newcommand{\DGDpara}   { \ensuremath{0.021 }}
\newcommand{\DGDperp}  { \ensuremath{0.012 }}
\newcommand{\DGDpS}   { \ensuremath{-0.011 }}
%

% G
\newcommand{\GAz}    { \ensuremath{-0.047 }}
\newcommand{\GApa}  { \ensuremath{-0.124 }}
\newcommand{\GAs}   { \ensuremath{0.156 }}
\newcommand{\GDpara}    { \ensuremath{-0.051 }}
\newcommand{\GDperp}    { \ensuremath{-0.017 }}
\newcommand{\GDpS}    { \ensuremath{0.019 }}
%

% Az
\newcommand{\AzApa}  { \ensuremath{-0.33}}
\newcommand{\AzAs}  { \ensuremath{0.216 }}
\newcommand{\AzDpara}    { \ensuremath{-0.019 }}
\newcommand{\AzDperp}   { \ensuremath{0.004 }}
\newcommand{\AzDpS}    { \ensuremath{0.014 }}
%

% Apa
\newcommand{\ApaAs}  { \ensuremath{0.056 }}
\newcommand{\ApaDpara}    { \ensuremath{0.201 }}
\newcommand{\ApaDperp}    { \ensuremath{0.058 }}
\newcommand{\ApaDpS}    { \ensuremath{-0.019 }}
%

% As
\newcommand{\AsDpara}    { \ensuremath{-0.094 }}
\newcommand{\AsDperp}    { \ensuremath{-0.012 }}
\newcommand{\AsDpS}  { \ensuremath{0.055 }}
%

% DeltaPara
\newcommand{\DparaDperp}    { \ensuremath{0.235 }}
\newcommand{\DparaDpS}    { \ensuremath{-0.014 }}
%
% DeltaPerp
\newcommand{\DperpDpS}    { \ensuremath{0.010 }}

% End of June 9 version  results %%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                                          SYSTEMATICS 9 June                     %%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pSsyst} { 0.036}
\newcommand{\DGsyst} { 0.007}
\newcommand{\GSsyst}  { 0.003}
\newcommand{\Apasqsyst} { 0.006}
\newcommand{\Azesqsyst} { 0.001}
\newcommand{\ASsqsyst}  { 0.013}
\newcommand{\Deltperpsyst} { 0.27} % was 0.25 before alignment
\newcommand{\Deltparasyst} { 0.05}
\newcommand{\DeltPSsyst}   { 0.01}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   END of Default fit    9 June version  %%%%%%%%% - version Bd 2.4%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
}


\newcommand{\sma}   { ${\small<}10^{-3}$} 
%
% End of "Replace following lines by extract from latex.tex fit results" 
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Alternative fits
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%%
% Bd up and down fits
%%%%%%%%%%%%%%%%%%%

\newcommand{\pSfitBdup}     {\ensuremath{-0.235}}
\newcommand{\pSstatBdup}    {\ensuremath{0.082}}
%

\newcommand{\DGfitBdup}     {\ensuremath{0.080}}
\newcommand{\DGstatBdup}   {\ensuremath{0.009}}
%

\newcommand{\GSfitBdup}    {\ensuremath{0.668}}
\newcommand{\GSstatBdup}    {\ensuremath{0.003}}
%

\newcommand{\ApasqfitBdup}    {\ensuremath{0.228}}
\newcommand{\ApasqstatBdup}  {\ensuremath{0.004}}
%

\newcommand{\AzesqfitBdup}    {\ensuremath{0.524}}
\newcommand{\AzesqstatBdup}    {\ensuremath{0.003}}
%

\newcommand{\ASsqfitBdup}     {\ensuremath{0.076}}
\newcommand{\ASsqstatBdup}     {\ensuremath{0.007}}
%

\newcommand{\DeltparafitBdup}    {\ensuremath{3.149}}
\newcommand{\DeltparastatBdup}    {\ensuremath{0.068}}
%

\newcommand{\DeltperpfitBdup}     {\ensuremath{4.678}}
\newcommand{\DeltperpstatBdup}    {\ensuremath{0.298}}
%
\newcommand{\DeltPSfitBdup}        {\ensuremath{-0.086}}
\newcommand{\DeltPSstatBdup}       {\ensuremath{0.030}}

% Bd down

\newcommand{\pSfitBddown}     {\ensuremath{-0.222}}
\newcommand{\pSstatBddown}    {\ensuremath{0.082}}
%

\newcommand{\DGfitBddown}     {\ensuremath{0.080}}
\newcommand{\DGstatBddown}   {\ensuremath{0.009}}
%

\newcommand{\GSfitBddown}    {\ensuremath{0.669}}
\newcommand{\GSstatBddown}    {\ensuremath{0.003}}
%

\newcommand{\ApasqfitBddown}    {\ensuremath{0.229}}
\newcommand{\ApasqstatBddown}  {\ensuremath{0.004}}
%

\newcommand{\AzesqfitBddown}    {\ensuremath{0.523}}
\newcommand{\AzesqstatBddown}    {\ensuremath{0.003}}
%

\newcommand{\ASsqfitBddown}     {\ensuremath{0.076}}
\newcommand{\ASsqstatBddown}     {\ensuremath{0.007}}
%

\newcommand{\DeltparafitBddown}    {\ensuremath{3.150}}
\newcommand{\DeltparastatBddown}    {\ensuremath{0.070}}
%

\newcommand{\DeltperpfitBddown}     {\ensuremath{4.671}}
\newcommand{\DeltperpstatBddown}    {\ensuremath{0.307}}
%

\newcommand{\DeltPSfitBddown}        {\ensuremath{-0.086}}
\newcommand{\DeltPSstatBddown}       {\ensuremath{0.030}}


%	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alternative fit with more pT Punzi time terms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\pSfitTimeAlt}     {\ensuremath{-0.194}}
\newcommand{\pSstatTimeAlt}    {\ensuremath{0.085}}
%

\newcommand{\DGfitTimeAlt}     {\ensuremath{0.099}}
\newcommand{\DGstatTimeAlt}   {\ensuremath{0.013}}
%

\newcommand{\GSfitTimeAlt}    {\ensuremath{0.678}}
\newcommand{\GSstatTimeAlt}    {\ensuremath{0.004}}
%

\newcommand{\ApasqfitTimeAlt}    {\ensuremath{0.230}}
\newcommand{\ApasqstatTimeAlt}  {\ensuremath{0.005}}
%

\newcommand{\AzesqfitTimeAlt}    {\ensuremath{0.520}}
\newcommand{\AzesqstatTimeAlt}    {\ensuremath{0.004}}
%

\newcommand{\ASsqfitTimeAlt}     {\ensuremath{0.102}}
\newcommand{\ASsqstatTimeAlt}     {\ensuremath{0.008}}
%

\newcommand{\DeltparafitTimeAlt}    {\ensuremath{3.147}}
\newcommand{\DeltparastatTimeAlt}    {\ensuremath{0.097}}
%

\newcommand{\DeltperpfitTimeAlt}     {\ensuremath{4.547}}
\newcommand{\DeltperpstatTimeAlt}    {\ensuremath{0.423}}
%

\newcommand{\DeltPSfitTimeAlt}        {\ensuremath{-0.082}}
\newcommand{\DeltSstatTimeAlt}       {\ensuremath{0.033}}


% End of Alternative fit with more pT Punzi time terms

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alternative fit with opening internal mass window for bg angles +-  85 MeV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\pSfitMassEightFiveAlt}     {\ensuremath{-0.201}}
\newcommand{\pSstatMassEightFiveAlt}    {\ensuremath{0.084}}
%

\newcommand{\DGfitMassEightFiveAlt}     {\ensuremath{0.097}}
\newcommand{\DGstatMassEightFiveAlt}   {\ensuremath{0.013}}
%

\newcommand{\GSfitMassEightFiveAlt}    {\ensuremath{0.678}}
\newcommand{\GSstatMassEightFiveAlt}    {\ensuremath{0.004}}
%

\newcommand{\ApasqfitMassEightFiveAlt}    {\ensuremath{0.229}}
\newcommand{\ApasqstatMassEightFiveAlt}  {\ensuremath{0.005}}
%

\newcommand{\AzesqfitMassEightFiveAlt}    {\ensuremath{0.521}}
\newcommand{\AzesqstatMassEightFiveAlt}    {\ensuremath{0.004}}
%

\newcommand{\ASsqfitMassEightFiveAlt}     {\ensuremath{0.104}}
\newcommand{\ASsqstatMassEightFiveAlt}     {\ensuremath{0.008}}
%

\newcommand{\DeltparafitMassEightFiveAlt}    {\ensuremath{3.148}}
\newcommand{\DeltparastatMassEightFiveAlt}    {\ensuremath{0.094}}
%

\newcommand{\DeltperpfitMassEightFiveAlt}     {\ensuremath{4.526}}
\newcommand{\DeltperpstatMassEightFiveAlt}    {\ensuremath{0.423}}
%

\newcommand{\DeltPSfitMassEightFiveAlt}        {\ensuremath{-0.080}}
\newcommand{\DeltSstatMassEightFiveAlt}       {\ensuremath{0.033}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alternative fit with opening internal mass window for bg angles +-  160 MeV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pSfitMasshundredsixtyAlt}     {\ensuremath{-0.201}}
\newcommand{\pSstatMasshundredsixtyAlt}    {\ensuremath{0.084}}
%

\newcommand{\DGfitMasshundredsixtyAlt}     {\ensuremath{0.100}}
\newcommand{\DGstatMasshundredsixtyAlt}   {\ensuremath{0.013}}
%

\newcommand{\GSfitMasshundredsixtyAlt}    {\ensuremath{0.680}}
\newcommand{\GSstatMasshundredsixtyAlt}    {\ensuremath{0.003}}
%

\newcommand{\ApasqfitMasshundredsixtyAlt}    {\ensuremath{0.230}}
\newcommand{\ApasqstatMasshundredsixtyAlt}  {\ensuremath{0.004}}
%

\newcommand{\AzesqfitMasshundredsixtyAlt}    {\ensuremath{0.519}}
\newcommand{\AzesqstatMasshundredsixtyAlt}    {\ensuremath{0.004}}
%

\newcommand{\ASsqfitMasshundredsixtyAlt}     {\ensuremath{0.100}}
\newcommand{\ASsqstatMasshundredsixtyAlt}     {\ensuremath{0.008}}
%

\newcommand{\DeltparafitMasshundredsixtyAlt}    {\ensuremath{3.148}}
\newcommand{\DeltparastatMasshundredsixtyAlt}    {\ensuremath{0.108}}
%

\newcommand{\DeltperpfitMasshundredsixtyAlt}     {\ensuremath{4.517}}
\newcommand{\DeltperpstatMasshundredsixtyAlt}    {\ensuremath{0.428}}
%

\newcommand{\DeltPSfitMasshundredsixtyAlt}        {\ensuremath{-0.079}}
\newcommand{\DeltSstatMasshundredsixtyAlt}       {\ensuremath{0.033}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% End of fit results for 2012
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\ifthenelse {\boolean{BdFraction3.3}}
{ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Combined results 2011 2012 for Bd3.3
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\pSfitCombi} { \ensuremath{-0.090} } 
\newcommand{\pSstatCombi} { 0.078 }
\newcommand{\pSsystCombi} { 0.041 }

%
\newcommand{\DGfitCombi} { 0.085 } 
\newcommand{\DGstatCombi} { 0.011 }
\newcommand{\DGsystCombi} { 0.007 }

%
\newcommand{\GSfitCombi} { 0.675 }
\newcommand{\GSstatCombi} { 0.003 }
\newcommand{\GSsystCombi} { 0.003 }

%
\newcommand{\ApasqfitCombi} { 0.227 }
\newcommand{\ApasqstatCombi} { 0.004 }
\newcommand{\ApasqsystCombi} { 0.006 }

%
\newcommand{\AzesqfitCombi} { 0.522 } 
\newcommand{\AzesqstatCombi} { 0.003 } 
\newcommand{\AzesqsystCombi} { 0.007 } 

%
\newcommand{\ASsqfitCombi} { 0.072 }
\newcommand{\ASsqstatCombi} { 0.007  }
\newcommand{\ASsqsystCombi} { 0.018 }

% 
\newcommand{\DeltperpfitCombi} { 4.15 }
\newcommand{\DeltperpstatCombi} { 0.32 }
\newcommand{\DeltperpsystCombi} { 0.16 }

%
\newcommand{\DeltparafitCombi}    { \Deltparafit }
\newcommand{\DeltparastatCombi}    { \Deltparastat }
\newcommand{\DeltparasystCombi}    { \Deltparasyst }

%
\newcommand{\DeltPSfitCombi}        { \DeltPSfit }
\newcommand{\DeltPSstatCombi}       { \DeltSstat }
\newcommand{\DeltPSsystCombi}       { \DeltPSsyst }
}
{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Combined results 2011 2012 for Bd2.4 - 9/6/2015
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pSfitCombi} { \ensuremath{-0.094} } 
\newcommand{\pSstatCombi} { 0.083 }
\newcommand{\pSsystCombi} { 0.033 }

%
\newcommand{\DGfitCombi} { 0.083 } 
\newcommand{\DGstatCombi} { 0.011 }
\newcommand{\DGsystCombi} { 0.007 }

%
\newcommand{\GSfitCombi} { 0.677 }
\newcommand{\GSstatCombi} { 0.003 }
\newcommand{\GSsystCombi} { 0.003 }

%
\newcommand{\ApasqfitCombi} { 0.227 }
\newcommand{\ApasqstatCombi} { 0.004 }
\newcommand{\ApasqsystCombi} { 0.006 }

%
\newcommand{\AzesqfitCombi} { 0.515 } 
\newcommand{\AzesqstatCombi} { 0.004 } 
\newcommand{\AzesqsystCombi} { 0.002 } 

%
\newcommand{\ASsqfitCombi} { 0.086 }
\newcommand{\ASsqstatCombi} { 0.007  }
\newcommand{\ASsqsystCombi} { 0.012 }

% 
\newcommand{\DeltperpfitCombi} { 4.13 }
\newcommand{\DeltperpstatCombi} { 0.34 }
\newcommand{\DeltperpsystCombi} { 0.16 }

%
\newcommand{\DeltparafitCombi}    { \Deltparafit }
\newcommand{\DeltparastatCombi}    { \Deltparastat }
\newcommand{\DeltparasystCombi}    { \Deltparasyst }

%
\newcommand{\DeltPSfitCombi}        { \DeltPSfit }
\newcommand{\DeltPSstatCombi}       { \DeltSstat }
\newcommand{\DeltPSsystCombi}       { \DeltPSsyst }
}



%%%%%%%%%%%%%%%%
% Selection cuts 
%%%%%%%%%%%%%%%%

%Jpsi

\newcommand{\cutMassJpsiBB} {$2.959\text{--}3.229$ \GeV}
\newcommand{\cutMassJpsiEB} {$2.913\text{--}3.273$ \GeV}
\newcommand{\cutMassJpsiEE} {$2.852\text{--}3.332$ \GeV}


\newcommand{\resMassJpsiBB} {$ 60 \pm 2 \MeV $}
\newcommand{\resMassJpsiEB} {$ 80 \pm 2 \MeV $}
\newcommand{\resMassJpsiEE} {$ 80 \pm 2 \MeV $}

\newcommand{\cutChiJpsi}   {\chisq $< 10$}

\newcommand{\NJpsi } {$ 75~\rm k$ \ }

% Bd
\newcommand{\cutpTKns}   {$ \psubt > 2.5 ~\rm \GeV $}
\newcommand{\cutMassKns} {$ (846-946) ~\rm \MeV $}
\newcommand{\cutChiBd}   {\chisq $< 2.5$}
\newcommand{\cutTauBd}   {$ \tau > 0.35 ~\rm ps $}

%Bs
\newcommand{\cutpTPhi}   {$ \psubt > 1.0 ~\rm \GeV $}
\newcommand{\cutMassPhi} {$ 1.0085 \; {\rm \GeV} < m(K^+ K^-) < 1.0305 \; {\rm \GeV} $}
\newcommand{\cutChiBs}   {\chisq $< 3$}
\newcommand{\cutTauBs}   {$ \tau > 0.4 ~\rm ps $}

%\newcommand{\cutMassBsmin}{$  5.2463 ~\rm GeV $}
%\newcommand{\cutMassBsmax}{$ 5.4863 ~\rm GeV $}

\newcommand{\cutMassBsRange}{ 5.150--5.650 \GeV}
%\newcommand{\cutMassBsLeftSide}{$  (5.2163- 5.317) ~\rm GeV $}
%\newcommand{\cutMassBsRightSide}{$  (5.417 -5.5163) ~\rm GeV $}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               2011 Results 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\DGfiteleven}     { 0.053 }	
\newcommand{\DGstateleven}    { 0.021 }
\newcommand{\DGsysteleven}    { 0.010 }

%
\newcommand{\pSfiteleven}     { 0.12 }	
\newcommand{\pSstateleven}    { 0.25 }
\newcommand{\pSsysteleven}    { 0.05 }

%
\newcommand{\GSfiteleven}     { 0.677 }	
\newcommand{\GSstateleven}    { 0.007 }
\newcommand{\GSsysteleven}    { 0.004 }
%
\newcommand{\Azesqfiteleven}     { 0.529 }
\newcommand{\Azesqstateleven}    { 0.006 }
\newcommand{\Azesqsysteleven}    { 0.012 }
%
\newcommand{\Apasqfiteleven}     { 0.220 }
\newcommand{\Apasqstateleven}    { 0.008 }
\newcommand{\Apasqsysteleven}    { 0.009 }
%
\newcommand{\ASsqfiteleven}      { 0.024 }	
\newcommand{\ASsqstateleven}     { 0.014 }
\newcommand{\ASsqsysteleven}     { 0.028 }
%
\newcommand{\Deltperpfiteleven}      { 3.89 }	
\newcommand{\Deltperpstateleven}     { 0.47 }	
\newcommand{\Deltperpsysteleven}     { 0.11 }
%
\newcommand{\Deltparafiteleven}     { [3.04, 3.23] }
%\newcommand{\Deltparastateleven}     { 0.09 } only interval given
\newcommand{\Deltparasysteleven}     { 0.09 }
%
\newcommand{\DeltPSfiteleven}        { [3.02, 3.25]}
%\newcommand{\DeltSstateleven}        { 0.04} only interval given
\newcommand{\DeltPSsysteleven}        { 0.04}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               LHCb 2011 Results combined Bs channels
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\DGfitcms}     { 0.095 }	
\newcommand{\DGstatcms}    { 0.013 }
\newcommand{\DGsystcms}    { 0.0073 }

%
\newcommand{\pSfitcms}     {- 0.075 }	
\newcommand{\pSstatcms}    { 0.097 }
\newcommand{\pSsystcms}    { 0.031 }

%
\newcommand{\GSfitcms}     {  0.670 }	% 
\newcommand{\GSstatcms}    { 0.005 }     % more precisely 0.004347
\newcommand{\GSsystcms}    {0.005   }   % 0.005096
%
\newcommand{\Azesqfitcms}     { 0.510  } 
\newcommand{\Azesqstatcms}    {0.005 }
\newcommand{\Azesqsystcms}    { 0.0114 }
%
\newcommand{\Apasqfitcms}     { 0.243 } 
\newcommand{\Apasqstatcms}    { 0.008 }
\newcommand{\Apasqsystcms}    { 0.0116  }
%
\newcommand{\ASsqfitcms}      { 0.012  }	
\newcommand{\ASsqstatcms}     { $^{+ 0.009} _ {- 0.007}$} % $^{+ } _ {- }$
\newcommand{\ASsqsystcms}     { 0.022 }
%
\newcommand{\Deltperpfitcms}      { 2.98  }	
\newcommand{\Deltperpstatcms}     {0.36 }	
\newcommand{\Deltperpsystcms}     { 0.66 }
%
\newcommand{\Deltparafitcms}     { 3.48 } 
\newcommand{\Deltparastatcms}     { $^{+ 0.07} _ {-  0.09}$  }
\newcommand{\Deltparasystcms}     { 0.685 }
%
\newcommand{\DeltPSfitcms}        { 0.37  }
\newcommand{\DeltSstatcms}        { $^{+ 0.28} _ {- 0.12}$  } 
\newcommand{\DeltPSsystcms}        {  0.18 }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               LHCb 2011 Results combined Bs channels
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\DGfitLHCbb}     { 0.100 }	
\newcommand{\DGstatLHCbb}    { 0.016 }
\newcommand{\DGsystLHCbb}    { 0.003 }

%
\newcommand{\pSfitLHCbb}     { 0.07 }	
\newcommand{\pSstatLHCbb}    { 0.09 }
\newcommand{\pSsystLHCbb}    { 0.01 }

%
\newcommand{\GSfitLHCbb}     { 0.663 }	
\newcommand{\GSstatLHCbb}    { 0.005 }
\newcommand{\GSsystLHCbb}    { 0.006 }
%
\newcommand{\AzesqfitLHCbb}     { 0.521 } 
\newcommand{\AzesqstatLHCbb}    { 0.006 }
\newcommand{\AzesqsystLHCbb}    { 0.010}
%
\newcommand{\ApasqfitLHCbb}     { 0.249  } % Aperp !!!!
\newcommand{\ApasqstatLHCbb}    { 0.009}
\newcommand{\ApasqsystLHCbb}    { 0.006 }
%
\newcommand{\ASsqfitLHCbb}      { - }	
\newcommand{\ASsqstatLHCbb}     { - }
\newcommand{\ASsqsystLHCbb}     { - }
%
\newcommand{\DeltperpfitLHCbb}      { 3.07 }	
\newcommand{\DeltperpstatLHCbb}     { 0.22 }	
\newcommand{\DeltperpsystLHCbb}     { 0.08 }
%
\newcommand{\DeltparafitLHCbb}     { 3.30 } 
\newcommand{\DeltparastatnegaLHCbb}     { \ensuremath{-0.21} } 
\newcommand{\DeltparastatposiLHCbb}     { + 0.13 }
\newcommand{\DeltparasystLHCbb}     { 0.08 }
%
\newcommand{\DeltPSfitLHCbb}        { - }
%\newcommand{\DeltSstatLHCbb}        { 0.04} only interval given
\newcommand{\DeltPSsystLHCbb}        {  - }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               LHCb 2011+2012 Results only BsJpsiKK
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\DGfitLHCbc}     { 0.0805 }	
\newcommand{\DGstatLHCbc}    { 0.0091 }
\newcommand{\DGsystLHCbc}    { 0.0032 }

%
\newcommand{\pSfitLHCbc}     { \ensuremath{-0.058} }	
\newcommand{\pSstatLHCbc}    {  0.049 }
\newcommand{\pSsystLHCbc}    {  0.006 }

%
\newcommand{\GSfitLHCbc}     { 0.6603 }	
\newcommand{\GSstatLHCbc}    { 0.0027 }
\newcommand{\GSsystLHCbc}    { 0.0015 }
%
\newcommand{\AzesqfitLHCbc}     { 0.5241 } 
\newcommand{\AzesqstatLHCbc}    { 0.0034 }
\newcommand{\AzesqsystLHCbc}    { 0.0067 }
%
\newcommand{\ApasqfitLHCbc}     { 0.2504 } % this is A perp!!! 
\newcommand{\ApasqstatLHCbc}    { 0.0049 }
\newcommand{\ApasqsystLHCbc}    { 0.0036 }
%
\newcommand{\ASsqfitLHCbc}      { - }	
\newcommand{\ASsqstatLHCbc}     { - }
\newcommand{\ASsqsystLHCbc}     { - }
%
\newcommand{\DeltperpfitLHCbc}      { 3.08 }	
\newcommand{\DeltperpstatnegaLHCbc}     { -0.15 }	
\newcommand{\DeltperpstatposiLHCbc}     { +0.14 }	
\newcommand{\DeltperpsystLHCbc}     { 0.06 }
%
\newcommand{\DeltparafitLHCbc}     { 3.26 } 
\newcommand{\DeltparastatnegaLHCbc}     { \ensuremath{-0.17} } 
\newcommand{\DeltparastatposiLHCbc}     { +0.10 }
\newcommand{\DeltparasystnegaLHCbc}     { -0.07 }
\newcommand{\DeltparasystposiLHCbc}     { +0.06 }
%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               LHCb 2011 Results only BsJpsiphi
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\DGfitLHCb}     { 0.116 }	
\newcommand{\DGstatLHCb}    { 0.018 }
\newcommand{\DGsystLHCb}    { 0.006 }

%
\newcommand{\pSfitLHCb}     { \ensuremath{-0.001} }	
\newcommand{\pSstatLHCb}    { 0.101 }
\newcommand{\pSsystLHCb}    { 0.027 }

%
\newcommand{\GSfitLHCb}     { 0.6580 }	
\newcommand{\GSstatLHCb}    { 0.0054 }
\newcommand{\GSsystLHCb}    { 0.0066 }
%
\newcommand{\AzesqfitLHCb}     { 0.523 }  
\newcommand{\AzesqstatLHCb}    { 0.007 }
\newcommand{\AzesqsystLHCb}    { 0.024}
%
\newcommand{\ApasqfitLHCb}     { 0.231 }  
\newcommand{\ApasqstatLHCb}    { 0.010}
\newcommand{\ApasqsystLHCb}    { 0.013 }
%
\newcommand{\ASsqfitLHCb}      { 0.022 }	
\newcommand{\ASsqstatLHCb}     { 0.012 }
\newcommand{\ASsqsystLHCb}     { 0.007 }
%
\newcommand{\DeltperpfitLHCb}      { 2.90 }	
\newcommand{\DeltperpstatLHCb}     {0.36 }	
\newcommand{\DeltperpsystLHCb}     { 0.07 }
%
\newcommand{\DeltparafitLHCb}     { [2.81 - 3.47] }  
%\newcommand{\DeltparastatnegaLHCb}     { -0.21 } 
%\newcommand{\DeltparastatposiLHCb}     { + 0.13 } 
\newcommand{\DeltparasystLHCb}     { 0.13 } 
%
\newcommand{\DeltPSfitLHCb}        {$\delta_S$= 2.90 } 
\newcommand{\DeltSstatLHCb}        { 0.36} 
\newcommand{\DeltPSsystLHCb}        {  0.08 }











%%%%%%%%%%%%%%%%%
% 2011 correlations 
%%%%%%%%%%%%%%%%%%

% phi - correlations

\newcommand{\pAzeleven}   {\ensuremath{0.002}}  %0.002 
\newcommand{\pApaeleven}  {\ensuremath{0.010}}   %0.010
\newcommand{\pAseleven}   {\ensuremath{ 0.029}}  %  0.029  
\newcommand{\pGeleven}    {\ensuremath{ 0.026}} %0.026 
\newcommand{\pDGeleven}   {\ensuremath{0.107}}   %0.107
 \newcommand{\pDparaeleven}   {\ensuremath{0.021}}
\newcommand{\pDperpeleven}   {\ensuremath{ -0.043}}
 \newcommand{\pDpSeleven}   {\ensuremath{ -0.003}}  %  $\delta_{\perp} -\delta_{S} $
%0.002      0.010       0.029        0.026   0.107 1.000 0.021 -0.043 -0.003

% DG
  
\newcommand{\DGAzeleven}  {\ensuremath{ 0.103}} % 0.103
\newcommand{\DGApaeleven} {\ensuremath{ 0.105}}   %0.105
\newcommand{\DGAseleven}  {\ensuremath{ 0.069}}  %0.069
\newcommand{\DGGeleven}   {\ensuremath{-0.617}} % -0.617
 \newcommand{\DGDparaeleven}   {\ensuremath{0.006}}
 \newcommand{\DGDperpeleven}   {\ensuremath{ -0.017}}
 \newcommand{\DGDpSeleven}   {\ensuremath{ 0.001}} %  $\delta_{\perp} -\delta_{S} $

% G
\newcommand{\GAzeleven}   {\ensuremath{-0.063}}  %-0.063
\newcommand{\GApaeleven}  {\ensuremath{-0.093}}  %-0.093
\newcommand{\GAseleven}   {\ensuremath{ 0.034}}  %0.034
 \newcommand{\GDparaeleven}   {\ensuremath{-0.003 }}
 \newcommand{\GDperpeleven}   {\ensuremath{ 0.001}}
 \newcommand{\GDpSeleven}   {\ensuremath{ -0.009}} %  $\delta_{\perp} -\delta_{S} $


% Az

\newcommand{\AzApaeleven} {\ensuremath{-0.316}} 
\newcommand{\AzAseleven}  {\ensuremath{ 0.283}}  
 \newcommand{\AzDparaeleven}   {\ensuremath{- 0.003}}
 \newcommand{\AzDperpeleven}   {\ensuremath{ -0.016  }}
 \newcommand{\AzDpSeleven}   {\ensuremath{ -0.025}} %  $\delta_{\perp} -\delta_{S} $

%Apa

\newcommand{\ApaAseleven} {\ensuremath{ 0.077}}  
\newcommand{\ApaDparaeleven}   {\ensuremath{0.008}}
 \newcommand{\ApaDperpeleven}   {\ensuremath{ 0.005}}
 \newcommand{\ApaDpSeleven}   {\ensuremath{ -0.010}} 

% As

\newcommand{\AsDparaeleven}   {\ensuremath{-0.011}}
 \newcommand{\AsDperpeleven}   {\ensuremath{  -0.054}}
 \newcommand{\AsDpSeleven}   {\ensuremath{ -0.098}} 

%Deltapara
\newcommand{\DparaDperpeleven}   {\ensuremath{ 0.038}}
\newcommand{\DparaDpSeleven}   {\ensuremath{ 0.007}} 
  
% Deptaperp
\newcommand{\DperpDpSeleven}   {\ensuremath{ 0.081}} 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                              End of  2011 Results 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%
%  LIfetime fits 
%%%%%%%%%%%%%%

\newcommand{\Bdtime}{$1.51\pm 0.04$}
\newcommand{\Bstime }{$1.41\pm 0.08$}

\newcommand{\Bdtimesta }{$1.51\pm 0.04~{\rm (stat)} \pm 0.04~{\rm (syst)}$}
\newcommand{\Bstimesta }{$1.41\pm 0.08~{\rm (stat)}\pm 0.05~{\rm (syst)}$ }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                               Results of mass only fits
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Bd

% before time cut
\newcommand{\Nsigdn} { $2680  \pm 150$ \ }
\newcommand{\Nbckdn} { $10280  \pm 110$ \ }
\newcommand{\Bdmassn} { $5278.6 \pm 1.3~\rm MeV$}
\newcommand{\mdresolutionn} { $36.8  \pm 2.0~\rm MeV$}
\newcommand{\scaledn} { $1.38  \pm 0.07$}

% before time cut Alastair - narrower window

\newcommand{\Nsigdnnar}{ $2440\pm 150$ \ }
\newcommand{\Nsigdnsnar}{ $2440\pm 150$ }
\newcommand{\Nbckdnnar}{ $9990 \pm 150 $ \ }
\newcommand{\Bdmassnnar}{ $5278.2   \pm 1.3 \  \rm MeV$}
\newcommand{\mdresolutionnner}{ $33.4 \pm 1.8 \  \rm MeV$}
\newcommand{\scaledmtnnar}{ $1.28 \pm 0.08$}


 \newcommand{\BdmassnnarNoMeV}{ $5278.2   \pm 1.3 \ $} 
 \newcommand{\mdresolutionnnerNoMeV}{ $33.4 \pm 1.8 \  $}
\newcommand{\BdmassnmtNoMeV}{ $5279.0 \pm 0.8$}
\newcommand{\mdresolutionnmtNoMeV}{ $34.3  \pm 0.9$}


% only m fit

\newcommand{\Nsigd} { $2340\pm 80$ \ }
\newcommand{\Nsigdns} { $2340\pm 80$ }
\newcommand{\Nbckd} { $1330 \pm 60 $ \ }
\newcommand{\Bdmass} { $5279.6   \pm 0.9 \  \rm MeV$}
\newcommand{\mdresolution} { $38.8 \pm 1.3 \  \rm MeV$}
\newcommand{\scaled} { $1.36 \pm 0.05$}

% With sta

\newcommand{\Nsigdsta} { $2340\pm 80~{\rm (stat)} $ \ }
\newcommand{\Nbckdsta} { $1330 \pm 60~{\rm (stat)} $ \ }
\newcommand{\Bdmasssta} { $5279.6   \pm 0.9~{\rm (stat)} \  \rm MeV$}
\newcommand{\Bdmassnsta} { $5278.6   \pm 1.3~{\rm (stat)} \  \rm MeV$}


\newcommand{\Bminmassd} { $5050   \  \rm MeV$ }
\newcommand{\Bmaxmassd} { $5550   \  \rm MeV$}
\newcommand{ \Bminmaxd}{ 5050--5550 MeV}


%%%%%%%%%%%%% Bs %%%%%%%%%%%%%%%%%%


% before lifetime cut

\newcommand{\Nsigsn} { $413 \pm 36$ \ }
\newcommand{\Nbcksn} { $764 \pm 17$ \ }
\newcommand{\Bsmassn} { $5363.6  \pm 1.6 \  \rm MeV$}
\newcommand{\msresolutionn} { $21.9 \pm 1.9 \  \rm MeV$}
\newcommand{\scalesn} { $1.08 \pm 0.09$ \ }


\newcommand{\BsmassnNoMeV} { $5363.6  \pm 1.6 \  $}
\newcommand{\msresolutionnNoMeV} { $21.9 \pm 1.9 \ $}
\newcommand{\BsmassNoMeV} { $5364.0 \pm 1.4 \  $}
\newcommand{\msresolutionNoMeV} { $26.6 \pm 1.5  \  $}



% after time cut
\newcommand{\Nsigs} { $358 \pm 22$ \ }
\newcommand{\Nsigsns} { $358 \pm 22$}
\newcommand{\Nbcks} { $90 \pm 7$ \ }
\newcommand{\Bsmass} { $5364.0 \pm 1.4 \  \rm MeV$}
\newcommand{\msresolution} { $26.6 \pm 1.5  \  \rm MeV$}
\newcommand{\scales} { $1.23 \pm 0.07$ \ }

\newcommand{\Nsigssta} { $358 \pm 22~{\rm (stat)}$ \ }
\newcommand{\Bsmasssta} { $5364.0 \pm 1.4~{\rm (stat)} \  \rm MeV$}
\newcommand{\Bsmassnsta} { $5363.6  \pm 1.6~{\rm (stat)} \  \rm MeV$ }
\newcommand{\Nbckssta} { $90 \pm 7~{\rm (stat)}$ \ }

\newcommand{\Bminmasss} { $5150   \  \rm MeV$}
\newcommand{\Bmaxmasss} { $5600   \  \rm MeV$}
\newcommand{ \Bminmaxs}{ 5150--5600 MeV}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                   Results of mass-time fit 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Bd

%before time cut
\newcommand{\Nsigdnmt}{ $2750  \pm 90$ \ }
%\newcommand{\Nbckdnmt}{ $9680  \pm 180$ \ }
\newcommand{\Nbckdnmt}{ $9680  \pm 310$ \ }
\newcommand{\Nbckdnmtnospa}{ $9680  \pm 310$ }
\newcommand{\Bdmassnmt}{ $5279.0 \pm 0.8~\rm MeV$}
\newcommand{\mdresolutionnmt}{ $34.3  \pm 0.9~\rm MeV$}
\newcommand{\scalednmt}{ $1.32  \pm 0.04$}



%after time cut (unchanged - original mass-only fit)

\newcommand{\Nsigdmt}{ $2340\pm 80$ \ }
\newcommand{\Nsigdnsmt}{ $2340\pm 80$ }
\newcommand{\Nbckdmt}{ $1330 \pm 60 $ \ }
\newcommand{\Nbckdmtnospa}{ $1330 \pm 60 $}

\newcommand{\Bdmassmt}{ $5279.6   \pm 0.9 \  \rm MeV$}
\newcommand{\mdresolutionmt}{ $38.8 \pm 1.3 \  \rm MeV$}
\newcommand{\scaledmt}{ $1.36 \pm 0.05$}

% With sta

\newcommand{\Nsigdstamt}{ $2340\pm 80~{\rm (stat)} $ \ }
\newcommand{\Nbckdstamt}{ $1330 \pm 60~{\rm (stat)} $ \ }
\newcommand{\Bdmassstamt}{ $5279.6   \pm 0.9~{\rm (stat)} \  \rm MeV$}
\newcommand{\Bdmassnstamt}{ $5279.0   \pm 0.8~{\rm (stat)} \  \rm MeV$}


\newcommand{\Bminmassdmt}{ $5159   \  \rm MeV$ }
\newcommand{\Bmaxmassdmt}{ $5399   \  \rm MeV$}
\newcommand{ \Bminmaxdmt}{ 5159--5399 MeV}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                                   Bs
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% before lifetime cut

\newcommand{\Nsigsnmt}{ $463 \pm 26$ \ }
%\newcommand{\Nbcksnmt}{ $714  \pm 16$ \ } 
\newcommand{\Nbcksnmt}{ $714  \pm 38$ \ } 

\newcommand{\Bsmassnmt}{ $5363.7  \pm 1.2$ \ }
\newcommand{\msresolutionnmt}{ $24.8 \pm 1.2$ \ }
\newcommand{\scalesnmt}{ $1.22 \pm 0.06$ \ }
\newcommand{\BsmassnmtMEV}{ $5363.7  \pm 1.2 \  \rm MeV$}
\newcommand{\msresolutionnmtMEV}{ $24.8 \pm 1.2 \  \rm MeV$}



% after time cut
\newcommand{\Nsigsmt}{ $349 \pm 16$ \ }
\newcommand{\Nsigsnsmt}{ $463 \pm 26$ \ }
%\newcommand{\Nbcksmt}{ ? }&////////
\newcommand{\Bsmassmt}{ $5362.2  \pm 1.3$}
\newcommand{\msresolutionmt}{ $27.0 \pm 1.4$}
\newcommand{\BsmassmtMEV}{ $5362.2  \pm 1.3 \  \rm MeV$}
\newcommand{\msresolutionmtMEV}{ $27.0 \pm 1.4  \  \rm MeV$}
\newcommand{\BsmassstamtMEV}{ $5362.2  \pm 1.3~{\rm (stat)} \  \rm MeV$}
\newcommand{\BsmassnstamtMEV}{ $5363.7  \pm 1.2~{\rm (stat)} \  \rm MeV$ }

\newcommand{\scalesmt}{ $1.26 \pm 0.07$ \ }

\newcommand{\Nsigsstamt}{ $349 \pm 16~{\rm (stat)}$ \ }
\newcommand{\Bsmassstamt}{ $5362.2  \pm 1.3~{\rm (stat)}$}
\newcommand{\Bsmassnstamt}{ $5363.7  \pm 1.2~{\rm (stat)}$ }
%\newcommand{\Nbcksstamt}{ ? }

\newcommand{\Bminmasssmt}{ $5150   \  \rm MeV$}
\newcommand{\Bmaxmasssmt}{ $5650   \  \rm MeV$}
\newcommand{ \Bminmaxsmt}{ 5150--5650 MeV}




%




% PDG

\newcommand{\Bspdg}       {$ 5.3663 \pm 0.0006 ~\rm GeV $}
\newcommand{\BspdgNoerr}  {$ 5.3663 ~\rm GeV $}
\newcommand{\Bdpdg}       {$ 5.2795 \pm 0.0003 \  \rm GeV $}
\newcommand{\Bstpdg}      {$ 1.472 \pm 0.026 ~\rm ps $}
\newcommand{\Bdtpdg}      {$ 1.525 \pm 0.009 ~\rm ps $}
\newcommand{\Bstpdgnops}  {$ 1.472 \pm 0.026 $}
\newcommand{\Bdtpdgnops}  {$ 1.525 \pm 0.009 $}
\newcommand{\Jpsipdg}     {$ 3096.916 \pm 0.011 ~\rm MeV $}
\newcommand{\Jpsipdgnoer} {$ 3096.916 ~\rm MeV $}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%                         DEFINITIONS

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%-----------------------------------------------------------------------  

% Bs JPsiphi specific
%\newcommand{\Bs}{\ensuremath{ B_{s}}\space} 
\newcommand{\Bst}{\ensuremath{ \Bs \ra \JpsiPhi }} 
\newcommand{\Bstbold}{\boldmath{ \Bs \ra \JpsiPhi }} 
\newcommand{\Bstn}{\ensuremath{ \Bs \ra \JpsiPhi}} 
\newcommand{\Bsto}{\ensuremath{ \Bs \ra J/\psi (\mumu) \phi(K^+K^-) }} 
\newcommand{\Bston}{\ensuremath{ \Bs \ra J/\psi (\mumu) \phi(K^+K^-) }} 
\newcommand{\Bdt}{\ensuremath{ \Bd \ra J/\psi K^{*} }} 

\newcommand{\BstoKK}{\ensuremath{ \Bs \ra J/\psi K^+K^- (f_{0}) }} 
%\newcommand{\Jpsi}{\ensuremath{ J/\psi }\space}
\newcommand{\JpsiPhi}{\ensuremath{ J/\psi\phi }} 
\newcommand{\JpsiPhin}{\ensuremath{ J/\psi\phi}} 
\newcommand{\JpsiPhito}{\ensuremath{J/\psi(\mumu) \phi(K^+K^-)  }} 

%\newcommand{\mumu}{\ensuremath{\mu^+ \mu^- }\space}

\newcommand{\aBst}{\ensuremath{ \aBs \ra \JpsiPhi    }} 
\newcommand{\Gs}{\ensuremath{ \Gamma_{s}     }}
\newcommand{\DGs}{\ensuremath{ \Delta\Gamma_{s}     }} 

\newcommand{\phis}{\ensuremath{\phi_{s}  }} 
\newcommand{\dms}{\ensuremath{\Delta m_{s}  }} 
\newcommand{\BH}{\ensuremath{B_{\rm H}  }} 
\newcommand{\BL}{\ensuremath{B_{\rm L}  }} 
%\newcommand{\GH}{\ensuremath{\Gamma_{H}  }\space} 
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}  }} 

\providecommand{\tildet}{\ensuremath{\tau}\xspace}
\providecommand{\sigtildet}{\ensuremath{\sigma_\tau}\xspace}

\providecommand{\tildeti}{\ensuremath{\tau_i}\xspace}
\providecommand{\sigtildeti}{\ensuremath{\sigma_\tau i}\xspace}
% Bd JpsipK0* specific

\newcommand{\BtoKns}{\ensuremath{  \Bo \ra  J/\psi  \Kns}\space}
\newcommand{\aBtoKns}{\ensuremath{  \aBo \ra  J/\psi \aKns}\space}
\newcommand{\BaBtoKns}{\ensuremath{  \BaBd \ra  J/\psi  \KaKns } }
\def\Kns{ \ensuremath{K^{   {*\rm \small 0}   }   } }
\def\aKns{ \ensuremath { \overline {K} ^{*\rm \small 0} } }
 \newcommand{\BaBd }{ \scalebox{1.}{$ \stackrel{\textrm{ \scalebox{0.7}[.5]{(---)} }}{\normalsize B^0}$} }
 
 
 \newcommand{\KaKns }{ \scalebox{1.}{$ \stackrel{\textrm{ \scalebox{0.7}[.5]{ (---)} }}{\normalsize \Kns }$}}
  
\newcommand{\BaBtoKnsto}{\ensuremath{ \BaBd \ra J/\psi(\mumu) \KaKns ( K^\pm \pi^\mp) } \space }
\newcommand{\BtoKnsto}{\ensuremath{ \Bo \ra J/\psi(\mumu) \Kns ( K^+ \pi^- ) } \space }


\newcommand{\JpsiKnsto}{\ensuremath{  J/\psi(\mumu) \KaKns ( K^\pm \pi^\mp) } \space }

\newcommand{\JpsiKnst}{\ensuremath{  J/\psi\Kns } \space }



\def \ra{\ensuremath{\rightarrow}}
\newcommand{\curlyL}{ \ensuremath{L}}
\newcommand{\GammaNeg}{\ensuremath {  \Gamma_{-} } \space} 
\newcommand{\ppFrac}{\ensuremath { pp_{fr} } \space}
\newcommand{\bbFrac}{\ensuremath { bb_{fr} } \space}
\newcommand{\mphi}{ \ensuremath { \phi }}
\newcommand{\Eff}{ \ensuremath { \epsilon }}
\newcommand{\wtf}{ \ensuremath { wf }}


%\newcommand{\bquark}{\ensuremath{b}}
\newcommand{\abquark}{\bbar  \space}

\newcommand{\bab}{\bbbar \space }
%\newcommand{\pp}{ pp   \space }
\newcommand{\cac}{ \ccbar} 
\newcommand{\bbJpsi}{\ensuremath{ \bbbar \ra  \Jpsi X  } \space}
\newcommand{\ppJpsi}{\ensuremath{ pp \ra \Jpsi X  } \space}

%Mesons

\newcommand{\Ds}{\ensuremath{D_{s}} \space} 
\newcommand{\BsaBs}{\ensuremath{\Bs} -- \ensuremath{\bar{B}^{0}_{s}}\space} 
%\newcommand{\BsaBs}{\ensuremath{\Bs - \aBs}} 
\newcommand{\B}{\ensuremath{B}\space  }
\newcommand{\aB}{\ensuremath{ \overline{\B}}\space} 



\newcommand{\Bo}{\ensuremath{ B^{0} }\space} 
\newcommand{\aBo}{\ensuremath{ \overline{B^{0}} }\space} 
\newcommand{\Bplus}{\ensuremath{ B^{+} }\space} 
\newcommand{\mBd}{\Bo\space} 
\newcommand{\mBs}{\Bs\space} 
\newcommand{\aBs}{\ensuremath{\bar{B}^{0}_{s}}} 
\newcommand{\aBsn}{\ensuremath{\overline{\Bs}}}
\newcommand{\bmass}{ \ensuremath{m(B)} \space}



% Upsilon(1S)
%\newcommand{\UoneS}{\ensuremath{\Upsilon(\mathrm{1S})}}
\newcommand{\Jpsipa}{\Jpsi \ }
\newcommand{\Jpsipan}{\Jpsi } 
\newcommand{\Upspa}{\Ups}
\newcommand{\jpsimass}{ \ensuremath{M (\Jpsipan) }\space}

\newcommand{\jpsieta}{ \ensuremath{\eta (\Jpsipan) }\space}
\newcommand{\jpsiphi}{ \ensuremath{\phi (\Jpsipan) }\space}
\newcommand{\jpsiPDGMass}{ \ensuremath{M_{PGD} (\Jpsipan) }\space}
\newcommand{\jpsiPDGmass}{ \ensuremath{M_{PGD} (\Jpsipan) }\space}
\newcommand{\jpsilxy}{\ensuremath{L_{xy} (\Jpsipan) }\space}
\newcommand{\lxyjpsi}{\ensuremath{L_{xy} (\Jpsipan) }\space}
\newcommand{\lxy}{\ensuremath{L_{xy} }\space}

\newcommand{\lxyb}{\ensuremath{L_{xy} (B) }\space}
                                                  
% pT
\newcommand{\psubt}{\pt \space} 

\newcommand{\jpsipt}{\pt (\Jpsipan) \space} 

\newcommand{ \ptb}{\pt (B) \space} 
\newcommand{ \bpt}{\pt (B) \space}
\newcommand{ \bdpt}{\pt (Bd) \space}
\newcommand{ \tauB}{ $\tau$ (B) \space}
% lumi
\newcommand{\lumilow}{\begL\   }
\newcommand{\lumimed}{\begM\   }
\newcommand{\lumihigh}{\lowL\   }
\newcommand{\lumihihh}{\highL\space} 
\newcommand{\pico}{\ipb\   }
\newcommand{\femto}{\ifb\space} 
\newcommand{\psubts}{\ensuremath{\pt > \GeV }\space} 
%\newcommand{\abseta}{\ensuremath{|\eta| }\space} 
\newcommand{\absetadp}{\ensuremath{\abseta < 2.4 }\space} 
\newcommand{\Hz}{\ensuremath{\rm Hz}\   }
\newcommand{\ps}{\ensuremath{\rm ps}\   }
%Statistics

\newcommand{\chisq}{$\rm \chi^{2}$/d.o.f. }


\newcommand{\Jpsitomm}{\ensuremath{ \Jpsi \ra \mumu }\space} 
\newcommand{\Jpsitoee}{\ensuremath{ \Jpsi \ra \epem}\space} 
\newcommand{\Jpsitol}{\ensuremath{\Jpsi \ra \mumu}\space} 
\newcommand{\mumuppi}{\ensuremath{\mumu p\pi^{-}}\space} 
\newcommand{\mueeppi}{\ensuremath{\mu eep\pi^{-}\ }\space} 
\newcommand{\bbarb}{\ensuremath{ pp \ra \bbbar X\ }\space} 
\newcommand{\phiKK}{\ensuremath{ \phi \ra \kplus \kminus}\space} 
\newcommand{\KnstoKpi}{\ensuremath{ \KaKns \ra K^{\pm}\pi^{\pm}\ }\space} 
\newcommand{\Kpi}{\ensuremath{ K^{\pm}\pi^{\mp}\space} \space} 
\newcommand{\Kpluspi}{\ensuremath{ K^{+}\pi^{-}}} 
\newcommand{\Kminuspi}{\ensuremath{ K^{-}\pi^{+}}} 

% B-decays
\newcommand{\btomu}{\ensuremath{\bbbar \ra  \mu\ X}\space} 
\newcommand{\bbJpsimumu}{\ensuremath{\bbbar \ra \Jpsitomm \ X}\space}
\newcommand{\ppJpsimumu}{\ensuremath{pp \ra \Jpsitomm \ X}\space}
\newcommand{\btomumu}{\ensuremath{\bbbar \ra  \mu^{+} \mu^{-} \ X}\space} 
\newcommand{\Bjpsi}{\ensuremath{ \B \ra \Jpsi }\space} 

% Others

\newcommand{\BstoDs}{\ensuremath{ \Bs \ra \Ds \pi  }\space} 
\newcommand{\BstoDsa}{\ensuremath{ \Bs \ra \Ds a_{1}  }\space} 
\newcommand{\Bsmumu}{\ensuremath{ \Bs \ra \mumu}\space} 

\newcommand{\BmumuKns}{\ensuremath{ \Bo \ra \mumu \Kns }\space} 
\newcommand{\Bplusmumuk}{\ensuremath{ B^{+} \ra \mumu \kplus }\space} 
\newcommand{\Bplusmmks}{\ensuremath{ B^{+} \ra \mumu K^{+*} (\kshort \pi^{+} ) }\space} 
\newcommand{\Kapluss}{\ensuremath{ K^{+*} \ra \kshort \pi^{+}  }\space} 
\newcommand{\Bsmumuphi}{\ensuremath{ \Bs \ra \mumu \phi }\space} 
\newcommand{\Lamzerobmumu}{\ensuremath{\Lamzerob \ra \mumu \Lamzero }\space} 
\newcommand{\Afbe}{\ensuremath{A_{FB}}\space} 
\newcommand{\bsdll}{\ensuremath{ b \ra s(d) l^+l^- \ }\space} 



\newcommand{\BtoKnsn}{\ensuremath{ \Bo \ra \Jpsi \Kns}\space} 

\newcommand{\BtoKpi}{\ensuremath{ \Bo \ra \Jpsi \kplus \piminus }\space} 
\newcommand{\BtoK}{\ensuremath{ \Bo \ra \Jpsi \kzero  }\space} 
\newcommand{\Bplust}{\ensuremath{ \Bplus \ra \Jpsi \kplus }\space} 
\newcommand{\bbJpsiX}{\ensuremath{ \bbbar \ra \Jpsi X  }\space} 
\newcommand{\bbJpsiXn}{\ensuremath{ \bbbar \ra \Jpsi X }\space} 
\newcommand{\ppJpsiX}{\ensuremath{ pp \ra \Jpsi X  }\space} 
\newcommand{\BplusJpsimumuKplus} {\ensuremath{B^{+} \ra \Jpsi(\mumu) \kplus }\space} 

\newcommand{\Lamzero}{\ensuremath{\Lambda^{0} }\space} 
\newcommand{\Lamzerob}{\ensuremath{\Lambda^{0}_{b} }\space} 
\newcommand{\Lamzeroto}{\ensuremath{\Lamzero \ra p \pi^{-} }\space} 
\newcommand{\LamzeroJpsi}{\ensuremath{\Lambda^{0} \Jpsi}\space} 
\newcommand{\Lamzerobto}{\ensuremath{\Lamzerob \ra \LamzeroJpsi }\space} 

\newcommand{\pb}{\ensuremath{pb^{-1}}}
\newcommand{\fb}{\ensuremath{fb^{-1}}}
\newcommand{\nb}{\ensuremath{nb^{-1}}}



%V
\newcommand{\Vubd}{\ensuremath{\Vub^{\ast} \Vud }\space} 
\newcommand{\Vcbd}{\ensuremath{\Vcb^{\ast} \Vcd }\space} 


\renewcommand{\thefootnote}{\fnsymbol{footnote}}


